Adaptive Memory Networks

We present Adaptive Memory Networks (AMN) that processes input-question pairs to dynamically construct a network architecture optimized for lower inference times for Question Answering (QA) tasks. AMN processes the input story to extract entities and stores them in memory banks. Starting from a single bank, as the number of input entities increases, AMN learns to create new banks as the entropy in a single bank becomes too high. Hence, after processing an input-question(s) pair, the resulting network represents a hierarchical structure where entities are stored in different banks, distanced by question relevance. At inference, one or few banks are used, creating a tradeoff between accuracy and performance. AMN is enabled by dynamic networks that allow input dependent network creation and efficiency in dynamic mini-batching as well as our novel bank controller that allows learning discrete decision making with high accuracy. In our results, we demonstrate that AMN learns to create variable depth networks depending on task complexity and reduces inference times for QA tasks.

==> abstract.tex <==
%\section*{Abstract}
\begin{abstract}
% Problem: Real world QA tasks, large number of tasks, hard to model and reason accurately 
% Solution: Adaptive Memory networks, learn to construct episodic memory based allowing low inference times to answer factual questions
% while higher inference times to answer questions more accurately or based on vague concepts/entity.

Real-world Question Answering (QA) tasks often consist of thousands of words that represent many facts and entities. Existing models based on LSTMs require a large number of parameters to support external memory and do not generalize efficiently for long sequence inputs. Memory networks address these limitations by storing information to an external memory module but must examine all inputs in the memory. Hence, for longer sequence inputs, the intermediate memory components proportionally scale in size, resulting in poor inference times. We present Adaptive Memory Networks (AMN) that process input-question pairs to dynamically construct a network architecture optimized for lower inference times.
AMN creates multiple {\em memory banks} that store entities from the input story to answer the questions. The model learns to {\em reason} important entities from the input text based on the question and concentrates these entities within a single memory bank. At inference, one or few banks are used, creating a tradeoff between accuracy and performance.
\toolshort\ is enabled by first, a novel bank controller that makes discrete decisions with high accuracy and second, the capabilities of a dynamic framework (such as PyTorch) that allow for dynamic network sizing and efficient variable mini-batching.  
In our results, we demonstrate that our model learns to construct a varying number of memory banks based on task complexity and achieves faster inference times by using fewer entities on tasks containing excess, unrelated information.
\end{abstract}
% \toolshort\ is enabled by first, a novel bank controller that makes discrete decisions using the reparameterization trick and second, the capabilities of dynamic framework (such as PyTorch) that allow dynamic network sizing and efficient variable mini-batching.  
% In our results, we demonstrate that our model learns to construct varying number of memory banks based on the task complexity and achieves faster inference times for toy tasks, standard bAbi tasks, and modified bAbi tasks. We achieve SOTA accuracy with (AVERAGE?\%) lower inference times.


%In this paper, we present adaptive short-term memory networks that train intermediate memory cells that are interpretable and can be 
%adaptively selected during inference. Given an input query, a small short-term working memory is constructed using activated representations 
%from within the long term memory using an iterative attention mechanism. An inference network is dynamically constructed using these memory cells, 
%using dynamic frameworks such as pytorch and an output is produced. We show benefits on language, program analyses and graph-based tasks.


==> app.tex <==
%all equations here

%\subsection{Loss}
%Loss is computed with cross entropy loss with added VAE loss for the memory bank controller's parameter estimation. $i,j$ are the two instances of an encoder and decoder in the memory bank controller.
%$$\mathcal{L}(\hat{\textbf{X}} \vert \theta, \phi ) = \text{CrossEntropy}(\hat{\textbf{X}}, \textbf{X}) - \sum_{i,j}\mathbb{E}_{\textbf{Z}~q_{\theta}(\textbf{Z}\vert \hat{\textbf{X}})}[\log p_{\phi} (\hat{\textbf{X}} \vert \textbf{Z})] +  \sum_{i,j}\sum q_{\phi}(\log q_{\phi} - \log(\frac{1}{2})))$$


%\renewcommand{\kbldelim}{(}% Left delimiter
%\renewcommand{\kbrdelim}{)}% Right delimiter
%\[
%  \text{N}_{n\text{ to }N} = \kbordermatrix{
%    & n_0 & n_1 & n_2 & n_3 & n_n \\
%    n_0 & 1 & 1 & 1 & 1 & 1 \\
%    n_1 & 0 & 1 & 0 & 0 & 1 \\
%    n_2 & 0 & 0 & 1 & 0 & 1 \\
%    n_3 & 0 & 0 & 0 & 1 & 1 \\
%    n_n & 0 & 0 & 0 & 0 & 1
%  }
%\]




%tldr AMN: \\
%task 1 all banks - 2.15 ms, passing - .6 ms\\
%task 2 all banks - 15.8 ms, passing - 3.2 ms\\
%task 7 all banks - 21 ms, passing - 6.0 ms\\

% \paragraph{Inference times}







==> intuition.tex <==
\subsection{Example Walkthrough}
\label{subsec:intuition}
Consider a toy example where our model is processing text input as sentences and a question to illustrate the adaptive inference of our model and how the memory bank controller (referred to as controller) is used. In the toy example, note how $s_2$ is unrelated to the question.
\begin{enumerate}
    \item $s_1:$ \texttt{John bought an apple.} $t=0$ 
    \item $s_2:$ \texttt{Mary walked to the office.} $t=1$
    \item $s_3:$ \texttt{John journeyed to the garden.} $t=2$
    \item $q_1:$ \texttt{Where is the apple?}
\end{enumerate}

$s_1$ is first processed by the encoder where each word is embedded into $\mathbb{R}^n$ (1). Then the accumulation GRU (4) learns the sentence states through time. In this instance, if $\textbf{u}_j$'s $wi_j$ is the word \texttt{an} where the previous states of \texttt{John, brought} will be contained in $\textbf{D}[\texttt{an}]$ and \texttt{an} has a record that \texttt{John, brought} has an association with itself. After the hidden states are computed, relevance strengths are learned w.r.t. $q_1$ (5-8), namely \texttt{apple} will have a high relevance score as it is mentioned in $q_1$. Nodes that are associated with \texttt{apple} will also have high scores. Lastly, a directed graph is drawn to contain the semantic information of $s_1$ where edges are drawn: $e(\texttt{John,brought}), e(\texttt{brought,an}), e(\texttt{an,apple})$ and stored in $\textbf{A}$. Note that the final hidden state for $s_1$ is equivalent to the hidden state of \texttt{apple}.

Once the prerequisite information for the nodes is encoded they are added into the memory $M$ with operation $\Pi_{au}$, specifically to the first memory bank $m_0$, the following operations are performed $\Pi_{new}$, $\Pi_{move}$. For $s_1$, the controller may learn not to create a new memory bank as the current state of $m_0$ does not contain enough information to reason through; subsequently $\Pi_{move}$ does not move entities. This concludes step $t=0$.

At $t=1$, $s_2$ is processed; the same initialization and metrics are computed and $s_2$'s nodes are added to the memory bank. However, as $s_2$ is wholly irrelevant to $q_1$, the nodes receive a low question relevance score. Now that new information is present, the controller now performs $\Pi_{au}$, $\Pi_{prop}$ before $\Pi_{new}$, $\Pi_{move}$. In $\Pi_{au}$, $s_2$'s nodes that are currently not present in $m_0$ are added. The hidden states of all nodes in $m_0$ are updated with the hidden state of $s_2$, \texttt{office} (15). The next hidden state updates occur under $\Pi_{prop}$ where nodes in connected components update their states according to incoming edges (16, 17). As there are more nodes in $m_0$ and the entropy is high, the controller decides to create a new memory bank $m_1$ and to duplicate move over question relevant nodes such as \texttt{John}, \texttt{apple}. The structure between \texttt{John}, \texttt{apple} is preserved and an edge is initialized between $e(\texttt{John},\texttt{apple})$. This concludes $t=1$.

%discuss how propagation works in more detail

For $t=2$, $s_3$ is initialized in the same manner but only the nodes \texttt{journeyed} and  \texttt{garden} are added to $m_0$ by $\Pi_{au}$. As this sentence has an association with \texttt{John} and thus \texttt{apple}, its nodes are given a higher weight. Edges are drawn from $e(\texttt{John}, \texttt{journeyed}), e(\texttt{journeyed}, \texttt{to}), e(\texttt{to}, \texttt{the}),  e(\texttt{the}, \texttt{garden}).$ Note, \texttt{the} has two outgoing edges to \texttt{office} and \texttt{garden}. The model begins by updating the states ($\Pi_{au}$) of the previous sentences with $s_3$'s hidden state, followed by propagation. This occurs in both $m_0, m_1$. Since $\Pi_{new}$ can only execute on the newest bank ($m_1$), it is skipped and $Pi_{move}$ is executed where the controller determines to bring \texttt{John}, \texttt{garden}, and \texttt{the} to $m_1$. As \texttt{John} already exists, only the last two nodes are carried over and their structures are preserved. Edges are drawn between \texttt{John} to \texttt{garden} and \texttt{the} as they are previously connected. Continuing onto $m_1$, the controller decides not to create a new memory bank as $m_1$ does not contain enough information.
%discuss how this works and the data structure used
Finally, we can see how throughout the memory module, the network has reasoned out the relevant entities (\texttt{John}, \texttt{garden}, \texttt{the}, \texttt{apple}). For the prediction, the model only considers $m_1$ and it's entities to construct an answer (18-21). It becomes evident that fewer entities are considered and thus fewer operations, saving on inference computations. 

% Currently at $t=0$, the only nodes that exist in memory are \texttt{John, bought, an, apple} First, the memory bank controller determines whether or not 
